Snowmass White Paper: New flavors and rich structures in dark sectors

Dark matter can be part of a dark sector with non-minimal couplings to the Standard Model. Compared to many (minimal) benchmark models, such scenarios can result in significant modifications in experimental signatures and strongly impact experimental search sensitivity. In this white paper, we review several non-minimal dark sector models, including phenomenological consequences: models explaining $(g-2)_\mu$, inelastic dark matter, strongly interacting massive particles as dark matter candidates, and axions with flavorful couplings. The present exclusions and projected experimental sensitivities on these example dark sector models illustrate the robustness of the growing dark sector experimental effort -- both the broadness and the precision of existing searches -- probing theoretically interesting parameter space. They also illustrate some of the unique complementarity of different experimental approaches.

==> Makefile <==
FILE=Snowmass_DMEFT

all: $(FILE).pdf

$(FILE).pdf : $(FILE).tex $(DIAS) DMEFT.bib figs/*
	pdflatex $(FILE).tex &&\
	bibtex $(FILE)       &&\
	pdflatex $(FILE).tex &&\
	pdflatex $(FILE).tex


clean:
	rm -vf *.dvi *.log *.aux *.bbl *.blg *.brf *.ilg *.toc *.out *.glo \
	  *.lof *.lot *.idx *.ind *.out *.fff *.ttt *.nlo *.nls



